R$^2$: A LLM Based Novel-to-Screenplay Generation Framework with Causal Plot Graphs

Automatically adapting novels into screenplays is important for the TV, film, or opera industries to promote products with low costs. The strong performances of large language models (LLMs) in long-text generation call us to propose a LLM based framework Reader-Rewriter (R$^2$) for this task. However, there are two fundamental challenges here. First, the LLM hallucinations may cause inconsistent plot extraction and screenplay generation. Second, the causality-embedded plot lines should be effectively extracted for coherent rewriting. Therefore, two corresponding tactics are proposed: 1) A hallucination-aware refinement method (HAR) to iteratively discover and eliminate the affections of hallucinations; and 2) a causal plot-graph construction method (CPC) based on a greedy cycle-breaking algorithm to efficiently construct plot lines with event causalities. Recruiting those efficient techniques, R$^2$ utilizes two modules to mimic the human screenplay rewriting process: The Reader module adopts a sliding window and CPC to build the causal plot graphs, while the Rewriter module generates first the scene outlines based on the graphs and then the screenplays. HAR is integrated into both modules for accurate inferences of LLMs. Experimental results demonstrate the superiority of R$^2$, which substantially outperforms three existing approaches (51.3%, 22.6%, and 57.1% absolute increases) in pairwise comparison at the overall win rate for GPT-4o.

==> documents/paper_zh.tex <==
% 中文版论文

\section{}{Introduction}

通用人工智能（AGI）的目标之一就是让模型能够像人类一样从事创造性的工作，最近大模型的兴起使得模型在故事生成、代码生成等文本生成任务上取得了媲美人类的能力。在这一背景下，剧本生成任务作为文本生成任务和评估人工智能系统创造性的一个重要子任务，在近年来也获得了大量关注\cite{zhuLeveragingNarrativeGenerate2022，mirowskiCoWritingScreenplaysTheatre2023, hanIBSENDirectorActorAgent2024}。

以前的剧本生成任务通过将一个故事提纲、叙事或概要扩写成一个完整剧本\cite{mirowskiCoWritingScreenplaysTheatre2023, hanIBSENDirectorActorAgent2024}在完成这一任务的过程中，模型（在完成这一任务的过程中）因为没有其它内容约束或参照，往往需要人类用户与模型进行大量的交互，并且输入的故事提纲、故事概要等也需要人类用户提供或者预设，这使得该任务对人类用户的参与度要求较高而对系统的自动化要求程度较低。

在本文中，我们提出了剧本生成任务的进阶版本——可控novel2script生成任务，该任务要求模型将给定的小说改编成剧本，在改编过程中人类的介入是可选的。这一任务的挑战性在于模型需要理解很长的小说文本并给出改编剧本；同时，模型改编的剧本应该前后一致并富有故事性，而且它应该保留所参照小说的主要情节。

该任务比以前的剧本任务更富有挑战性。虽然生成式模型的上下文窗口大小正不断提高，但是一次性阅读一本小说对于当前的主流大模型如GPT-4来说还是非常困难的，而且在处理长文本过程中这些大模型还是会出现long-range dependencies问题\cite{大模型的长文本生成问题}，生成的故事文本往往会出现前后不一致，因此这一任务可以作为AGI系统智能程度的试金石。

此外，这一任务的应用价值和研究意义也是很明显的。将现有的热门小说和已有的经典小说自动改编成剧本将极大降低影视行业的制作成本，辅助影视行业传播这些作品，从而有效提升这些小说的传播度和知名度。并且，研究这一任务还有助于开发更加实用的文本生成系统和视频生成系统，搭配成熟的剧本改编系统和视频生成系统，未来AI将能够全自动地将一部小说拍成影视剧\cite{zhuMovieFactoryAutomaticMovie2023}，这对于开发具有创造性的AGI系统有重要意义。

现有的剧本生成和故事生成方法大部分都是直接用GPT-4等通用大模型将小说对应章节直接改编成剧本，但是这样的方法未考虑引入剧本的各种结构和情节、人物、场景等关键要素的控制和改编，无法保证改编的剧集情节前后一致，而且还会有角色信息出现前后不一的情况（例如出现角色情节错乱\cite{yangRe3GeneratingLonger2022}）。
另外，尽管大模型的上下文窗口正不断扩大，但是由于小说的篇幅太大，这些小说仍然难以被大模型一次性处理和理解\cite{大模型的阅读理解问题}。因此，如何使模型能够有效理解长文本并保证模型改编的剧集具有一致性和连贯性成为解决这一任务的关键。

从人类剧作家基于小说改编剧本的一般过程（思路）中，我们获取了解决这一挑战的方法。我们观察到，剧作家在改编剧本时并非照着小说将小说逐章改编成剧本，他们首先会作为一个读者反复地阅读小说，从原小说中提炼出主次要情节和主次要人物，然后再依据这些信息写出改编剧本的大纲，并依据大纲和原小说中的人物对话逐条编写出原始剧本，最后在对原始剧本和大纲进行反复（讨论）修改之后，剧作家会交付最终的剧本\cite{剧本创作理论}。因此，在这一过程中，对原小说的阅读提炼和改编剧本大纲的编写是决定剧作家改编质量的关键。

Inspired by such ideas，我们提出了以情节图为中心的Reader-Rewriter框架，该框架将关注点放在对小说情节图的提炼和改编上。我们将情节视为一个个事件组成的有向无环图（即plot graph），我们的方法用一个基于LLM的Reader提取包括人物经历、情节图和场景地点等在内的戏剧关键元素用于剧本改编。具体来说，我们首先将小说章节分成若干段输入一个基于滑动窗口思想设计的大模型逐章提取模块，该模块依据先前提取的情节图等元素和后续章节，将小说当前的若干章节的内容提取为一个章节情节图。然后，我们通过Issues-aware self-refine模块将这些相关性较差的章节情节图进一步优化完善为一个整体的小说情节图。

接下来，我们的Rewriter将基于小说情节图对小说情节进行改编并完成剧本生成。在这个过程中，Rewriter将改写小说的情节图形成剧本的情节大纲、改写人物经历和故事线、设定场景目标以确定整个剧本结构的outline，最终Rewriter基于这些信息生成最终剧本中的每一个scene从而完成整部剧本的生成。

通过这种方式，我们的生成框架能够获取到一个完整反映整个小说内容的连贯的情节大纲，并依据这个大纲将小说改编成一个连贯的剧本。

为了评估我们生成的剧本质量，我们收集了xxx数据作为测试数据集，并设计了基于GPT-4的自动评估方法和基于Likert五点量表的人工评估方法，我们将GPT-4和其它剧本生成工具作为我们的baseline进行比较。**具体的实验结果总结。**

We summarize our contributions as follows:
1. 我们提出了一个适用于可控剧本生成任务的以情节图为中心的可控novel-to-script框架R2，该框架能通过LLM获取一个完整反映整个小说内容的连贯的情节大纲，并通过改编这个大纲将原小说改编为一个情节链连贯的剧本。
2. 我们在R2的设计中提出了针对长文本处理的滑动窗口技术和issue-aware contextual self-refine技术，并在提取情节链和生成场景时引入了连贯性判别模块，这些技术能帮助我们准确地提取出情节链和人物profile，并将情节链和人物profile有效地改编成剧本大纲，从而提升剧本生成的质量。
3. 我们收集了xxx数据作为测试数据集，并设计了基于GPT-4的自动评估方法和基于Likert五点量表的人工评估方法用于评估我们的方法。结果表明，我们的R2框架能生成质量远超于baseline的剧本，这进一步证明了R2框架的有效性，并为未来的可控novel-2-script生成工作提供了新的基准。

\section{Related Work}

**Long-form Generation** 近年来，随着LLM的出现和发展，长文本生成领域涌现出了许多工作。其中很多工作都致力于解决长文本生成中的long-range dependency问题和生成内容的long-range plot coherence, premise relevance, and  factual consistency的挑战。**Plan-and-Write** \cite{}提出了一个计划和编写的分层生成框架，该框架结合了情节规划和基于情节的自然语言生成从标题生成故事。Re3 \cite{}通过将生成过程分解为plan、draft、rewrite、edit四个阶段，并采用**Recursive** **Reprompting** **and Revision**的方式从给定的premise开始逐步生成故事大纲和最终的故事。**DOC** \cite{}提出一个分层大纲生成框架，将细纲的每一项都与相关人物联系起来提升整体连贯性，基于FUDGE实现了一个控制器加强对段落的可控生成。**Ex3** \cite{}提出一个三步微调生成框架，它先从原始小说库中提取结构信息，然后用提取的信息构建指令数据集微调LLM增强其谋篇布局的能力，最后用树状分层生成的结构将前提展开为小说。

另外还有一些工作专注于构建生成剧本的模型和人机交互框架。ScriptWriter \cite{}第一次对基于叙述的电影剧本对话选择任务进行研究并提出了一个考虑叙述的生成模型框架。Dramatron \cite{}提出一个分层故事生成的方法，它用提示链提示LLM根据log line分层生成剧本所需的人物、情节、location等关键元素，并根据这些元素生成场景对话，最终将这些内容组合成剧本，在这个生成过程中人类用户通过与LLM交互能够协作生成情节连贯的长剧本。IBSEN \cite{}提出一个多智能体架构，使得用户能够通过导演-人物多智能体互动完成可控剧本生成。**MovieFactory** \cite{}通过多种提示从输入文本出发构建起电影场景描述用于生成最终的电影视频。

% 这些工作不同，我们的方法面向CNSG任务，它既要求模型理解长文本小说，又要能够自动生成情节连贯的高质量改编剧本。
与这些工作相比，我们的方法面向CNSG任务，它既要求模型理解长文本小说，又要能够自动生成情节连贯的高质量改编剧本。因此我们的方法需要解决理解和生成长文本两方面的问题。

**LLM-Based Self-Refine Approach**  迭代式自我完善是人类解决问题的基本特征\cite{}。正如作家、编剧等文本创作者可以通过不断修改自己创作的草稿来使自己的作品更臻完美，作为文本生成器的LLM也可以通过不断地self-refine进一步改进自己生成的质量\cite{}。在之前的工作中，Self-critiquing \cite{}和\citet{} 通过采用自然语言反馈对LLM进行微调精炼改进LLM在summary任务上的表现。Reflexion \cite{}使用verbal reinforcement 的强化学习方法帮助LLM从先前的失败中学习和self-refine自己的输出。LLM-Augmenter \cite{}使用一个即插即用模块通过外部知识和自动反馈来改进 LLM。Self-Refine\cite{}证明了LLM通过自我提示就能改进自己在多个生成任务中所犯的错误。

在本文中我们的精炼方法主要参考基于LLM自我提示的self-refine方法，同时也改进了self-refine的基本方法用于解决情节图提取和长文本生成问题。

Approach（Reader-Rewriter）

overview

如图所示\ref{}，我们的Reader-Rewriter框架主要由两部分构成，基于LLM的Reader和基于LLM的Rewrter，前者用于从小说中提取情节图和人物经历，后者用于根据小说情节图和人物经历将小说改编成剧本。为了从长文本小说中提取出准确连贯的情节图和人物经历，我们在LLM-Based Reader引入了滑动窗口提取、issue-aware self-refine以及情节图检测等方法，接下来的Sec. \ref{}将介绍LLM-Based Reader中使用的这些方法。为了从情节图和人物经历出发生成最终的剧本，我们首先利用LLMs提出改编剧本的计划，包括情节大纲、剧本结构、每一个scene的故事线和目标，然后再根据情节图获取的Scene-aware Context和上述改编计划生成每一个scene的剧本，最后对scene的剧本进行self-refine从而完成最终版剧本的生成。接下来的Sec. \ref{}将介绍LLM-Based Rewriter生成剧本的过程。

### LLM-Based Reader

*书读百遍，其义自现 ————朱熹 \cite{}*

人类阅读小说时，经常会逐章梳理小说情节和人物关系并与前后章的上下文情节联系起来从而形成对整部小说的认识，认识的结果往往可以用一个图的方式展现出来。并且这个认识过程往往是渐进的，也就是说，由于小说篇幅往往很长，人们并非一次读完整部小说就能完全理解章节之间的情节联系和人物关系，他们往往是要经过多次阅读总结梳理之后才能完全熟悉整个小说的主题思想、故事结构和主要内容，从而能将这些内容展现成一个完整的情节图。同时，以前的文本摘要工作中也经常使用分层框架来逐步提取出整个文本的重要信息\cite{}。

% 受这一过程的启发，我们设计了LLM-Based Reader的基本处理模块，它们分别是基于滑动窗口的章节理解模块和基于self-refine的理解优化模块。前者用于构建一个初始的章节情节图和人物经历，后者则将这些初始的理解内容扩展为关于整部小说的情节图和人物经历。
% TODO：这里要修改
受这一过程的启发，我们设计了LLM-Based Reader的基本处理模块，它们分别是基于滑动窗口的章节理解模块和基于self-refine的理解优化模块。前者用于构建一个初始的章节情节图和人物经历，后者则将这些初始的理解内容扩展为关于整部小说的情节图和人物经历。

\paragraph{The Plot Graphs and Character Arcs} 
情节图能够有效表示故事的结构和事件关系。\citep{}最早提出plot graphs的概念，他将plot graphs定义为
The plot graph first presents modeling the author's intended logical flow of events in the virtual world as a set of precedence constraints between plot events \citet{weyhrauch1997guiding}，后来\citet{liStoryGenerationCrowdsourced2013} 将plot graph定义为一个图结构，其中图的顶点表示情节事件，图的边表示ordered pairs of events with precedence constraints，此外情节图中还包含a set of unordered mutual exclusion relations which restrict certain events from co-occurring in the same narrative.
在本文中，我们将情节定义为事件之间的因果关系，情节图是一个描述事件及事件间的因果关系的有向无环图，它的数学定义如下：G=<E,D,W>, E表示由时间地点和event description组成的事件，D表示事件之间存在的因果关系描述，W表示因果关系D的强度，由low，middle，high三个等级构成。
人物关系和人物经历是生成故事的另外一个重要元素\citep{}，为了从小说中提取出有助于理解人物的信息从而辅助将小说改编成剧本，我们将人物弧线定义为人物关系和人物小传的二元组，其中人物关系R是一个无向图<C，R>，C表示人物名称，R表示人物关系的描述；人物小传是不同角色经历的各种事件和心理变化的集合。
Reader的目标就是提取出小说对应的情节图结构和Character Arcs从而帮助我们基于这些信息进一步将小说改编成剧本。

\paragraph{人物事件提取模块} 关于滑动窗口
为了提取出情节图，我们首先需要提取小说的情节事件。在Chapter Extraction Module中，由于LLMs的输入上下文窗口有限，我们要求LLMs按章节提取情节事件，这里我们要求LLMs为我们提取如图\ref{}所示的事件元素，包括Diegesis，Description，Place and Time，Detailed，Associated Characters，这可以通过要求LLM生成结构化的输出来实现\citep{}。在提取事件时我们发现，如果LLMs只按照每一章的内容提取相应事件，从相邻章节中提取出的事件之间可能会存在不一致，最终这种错误累积最终可能会导致严重的情节事件偏差。为了降低这种不一致带来的偏差，我们通过滑动窗口技术提取当前章节的事件，具体来说就是在生成当前章节时，我们将之前提取的事件和滑动窗口内的后续章节内容作为上下文提供给LLMs并要求它尽量提取出一致的情节事件。同时，我们也通过相同的方法提取出每一章的Character Arcs。具体过程如图所示\ref{},经过这一步后，我们提取出章节对应的情节事件和和Character Arcs。
% 这是因为提取时未考虑当前窗口的小说上下文内容，
% 我们使用滑动窗口技术通过LLMs提取当前输入窗口内的情节事件，这里我们要求LLMs为我们提取如图\ref{}所示的事件元素，包括Diegesis，Description，Place and Time，Detailed，Associated Characters，这可以通过要求LLM生成结构化的输出来实现\citep{}。在提取事件时我们发现，如果LLMs对当前输入窗口的内容进行事件提取，则从相邻窗口中提取出的事件之间可能存在不一致，这是因为提取时未考虑当前窗口的小说上下文内容。为了保证提取的一致性
% \paragraph{人物事件优化模块} 在提取时
然而，在提取出章节对应的情节事件和和Character Arcs时，我们发现LLMs会出现幻觉现象：小说中的有些事件和Character Arcs仍然没有提取出来，并且提取出来的这两者之间还存在着不一致。为了减轻LLMs的这一问题，我们基于self-refine\citep{}的思想要求LLMs对事件、人物弧线的提取不完整以及事件-人物弧线之间的不一致分别进行循环self-refine，直到事件和Character Arcs都提取完整并且事件、Character Arcs之间保持一致。同时，为了提升LLM在根据self-refine的问题定位和建议修改相应事件、Character Arcs的针对性，我们设计了issue-aware self-refine。具体来说，如图所示\ref{},在每一轮根据LLMs给出的反馈改善对事件和Character Arcs的提取结果时，我们根据反馈的错误定位只获取提取结果中的错误部分以及相关的章节上下文输入给LLMs并要求它进行self-refine，并将最终改进的结果合并到整体的提取结果中进行下一轮的LLMs反馈获取。经过对人物事件的issue-aware self-refine后，我们将得到更加全面地涵盖整部小说内容并且更加一致的事件和Character Arcs。
% 同时，考虑到LLM在进行self-refine的过程中在寻找问题和优化的时候参考的上下文长度可能超过LLMs的最长输入限制，

% 关系强度很低的不正确
\paragraph{情节图构建模块} 
% 关于建图破圈  
在提取完事件和character arcs之后，我们利用这些提取内容进一步构建情节图。首先我们指示LLMs提取事件之间的关系，事件之间的关系主要包括对关系的描述和关系强度。这里我们用low，medium，high三个等级描述事件的因果关系强度。由于LLMs通常无法一次提取所有关系，我们通过将之前提取的关系作为上下文提示LLMs完成多轮关系提取。最终直到关系提取数量趋于稳定之后，我们得到了一个初始的情节图。
然而，在初始的情节图中，由于LLMs的幻觉，这个图中往往存在环和各种实际上不存在因果关系的事件关系。为了去除图中的环和错误提取的事件关系，我们采用一种破环prim算法的变体，如算法\ref{}所示，它主要基于关系强度和事件节点的度数进行破环,破环过程中我们优先保留因果关系强和节点度数越小的关系-事件图,从而保证最终得到的DAG中去掉了不重要的边，同时保留了足够重要的关系和事件使得图整体上连通。
% 它主要将因果关系强弱为第一关键字，节点度数为第二关键字进行破环，

\begin{algorithm}[ht]
\label{alg1}
\caption{Greedy Cycle-Breaking Algorithm for Directed Acyclic Graph (DAG)}
\KwIn{A set of events $plot\_lines$ and causal edges $plots\_edges$}
\KwOut{A set of edges $final\_edges$ forming a DAG}

\textbf{Step 1: Initialize Degree and Reachability Sets}
\begin{itemize}
    \item Extract event IDs from $plot\_lines$.
    \item Initialize the degree of each event to zero.
    \item Initialize two sets for each event:
    \begin{itemize}
        \item $to[event]$: the set of events reachable from this event (initially just the event itself).
        \item $fr[event]$: the set of events that can reach this event (initially just the event itself).
    \end{itemize}
\end{itemize}

\textbf{Step 2: Sort Edges by Priority}
\begin{itemize}
    \item Assign a priority to each edge based on the strength of its causal relationship: HIGH, MEDIUM, LOW.
    \item Sort edges by:
    \begin{enumerate}
        \item Causal strength (HIGH priority first).
        \item Sum of degrees of the two events connected by the edge (lower degree has higher priority).
    \end{enumerate}
\end{itemize}

\textbf{Step 3: Add Edges Greedily to Avoid Cycles}
\begin{itemize}
    \item For each edge $(a, b)$ in sorted order:
    \begin{itemize}
        \item If adding $(a, b)$ creates a cycle (i.e., $b$ is already reachable from $a$), skip this edge.
        \item Otherwise, add the edge and update the reachability sets:
        \begin{itemize}
            \item Add all reachable nodes from $b$ to all predecessors of $a$.
            \item Add all predecessors of $a$ to all reachable nodes from $b$.
        \end{itemize}
    \end{itemize}
\end{itemize}

\textbf{Step 4: Return Final Edge Set}
\begin{itemize}
    \item Return $final\_edges$, which now forms a directed acyclic graph (DAG).
\end{itemize}

\end{algorithm}


### LLM-Based Rewriter

the only kind of writing is rewriting ————Hemingway \cite{}

编剧改编剧本时常常要先列出一个剧本大纲，其中包含了改编剧本的主题、故事线和主要人物关系。在确定了这些改编剧本的关键要素之后，编剧还要选择一个合适的剧本框架如著名的三幕式（开头、中间和结尾）、弗雷塔格金字塔（阐述、煽动事件、由一系列冲突、并发症和困境组成的上升动作、高潮、坠落动作、解决和结局）将剧本大纲转换成每一个act和scene的具体写作提纲。确定了这些之后，编剧才开始依照这些提纲对每一幕的内容不断的改写以完成剧本创作。先前的各种长文本生成工作也都证明了先列提纲再写作这种范式对长文本生成的有效性。

因此，我们根据上述过程设计了LLM-Based Reader的基本处理模块，包括情节图改编模块和基于self-refine的剧本生成模块。前者用于将小说情节图改编成合适的剧本写作提纲，后者根据剧本写作提纲生成每一个scene的剧本并对这些剧本不断修改以得到最终的剧本。

% 我们需要考虑用何种顺序展示情节图给LLMs。正如有向无环图有两种遍历方式深度优先遍历和广度优先遍历一样，我们的情节图加上原始的存储方式以 不同模式对LLMs改编剧本的影响 关于情节图改编
\paragraph{改编大纲生成模块} 
获得情节图和人物弧线之后，我们考虑基于它们制定一个剧本改编大纲。剧本改编大纲由Story Core Elements， Screenplay Structure， Adapted Acts List以及组成幕的每一个Scene的写作计划组成，如图所示\ref{}。首先我们指示LLMs基于情节图和人物弧线按顺序生成这些剧本改编大纲的关键元素，在生成改编大纲时我们发现这些元素尤其是scene的写作计划经常出现事件和人物之间的问题，因此在提取出初始的剧本改编大纲之后我们还需要再提示LLMs对剧本改编大纲进行self-refine，在这里我们主要关注对关键场景和主要人物的改编。经过几轮self-refine之后我们得到最终版本的改编大纲。
这里有一点值得注意的是，在生成大纲的过程中，我们的情节图有三种展示的方式，包括深度优先遍历、广度优先遍历和原始章节顺序的展示方式。这三种方式分别代表了从主线出发改编剧本、从事件发生先后出发改编剧本和按照原小说写作顺序改编剧本这三种模式，因此我们对不同的情节图展示方式进行了实验分析，实验结果将在Sec. \ref{}中描述。

\paragraph{剧本生成模块} 关于剧本生成

获取改编大纲之后，我们开始基于大纲中对于每个scene的写作计划对每个scene进行实际写作。scene的写作计划包括写作故事线，storyline goal, place and time，character experiences。仿照Sec. \ref{}的事件提取方式，我们每提示LLM生成一个scene时都会从与写作计划相关联的小说原始章节中获取相关片段以及前一个生成的scene作为上下文输入给LLMs，这样做使得我们生成的剧本scene之间能够保持一致性，同时与小说的相关情节保持一致。另一方面，我们在生成了每一个scene之后还会提示LLMs进行self-refine以检查生成的scene是否达到了故事线目标，从而保证每个scene都能遵照写作大纲，保证每个scene都能达到改编要求。

总的来说，我们生成的过程与阅读理解的过程在high level上正好是相反的，按照\citet{}, 这保证了我们的改编框架能够依照对原小说的理解生成可控性强的改编剧本。

# Experiment

## Experimental Setting

\paragraph{Task Setup} 我们的方法能够通过给定一个小说生成一部完整的剧本。为了评估我们方法的有效性，我们通过给定一个相同的小说来比较由R2方法和其它baseline方法生成的剧本。我们的R2框架采用7B大小的GPT-4o-mini版本\footnote{\url{https://platform.openai.com/docs/models/gpt-4o-mini}}作为我们的基座模型，其它基线采用原始方法相应的LLMs。

\paragraph{Datasets Construction} 为了评估我们方法的生成效果，我们从一些公开网站\footnote{\url{https://www.gutenberg.org/}, \url{https://manybooks.net/}, \url{https://digilibraries.com/}, \url{https://8flix.com}, \url{https://www.scriptslug.com}}搜集了小说改编电影的小说-剧本对通过人工清洗构建我们的评估数据集。同时，考虑到GPT-4在训练时可能用到了这些电影的剧本或者小说作为训练语料，其中与热门电影相关的语料更多，与冷门电影相关的语料更少\citep{}，这使得GPT对这些电影、剧本的了解程度不同，因此我们根据小说改编电影的评分、观看人数将我们收集的这些小说-剧本对分为冷门和热门电影数据集，用于检测我们的方法在GPT了解程度不同的小说上进行剧本改编的效果。另外，我们选取了3个小说-剧本对作为验证集用于测试调整我们的方法。这些数据集的基本信息如Table \ref{}所示。

\paragraph{Evaluation Methods} On the one hand, following prior work like Re3\citep{} and DOC\citep，我们通过设计调查问卷并将其提交给评估人员进行评分，对我们的方法和各个baseline进行成对实验。问卷由一个原始小说选段、两个剧本选段（记为A和B，顺序随机）和一组问题组成。问卷的问题针对**Interesting**: Captivates the reader’s attention；**Coherent**: The plot flows smoothly, and the scene changes are not abrupt；**Human-like**: Natural language resembling human writing；**Diction and Grammar**: Accurate word choice and elegant grammar；**Transition**: Smooth and natural rhythm of the story and the emotional changes of the characters；**Script Format Compliance**: Adheres to standard script formatting rules；**Consistency**: Consistent with the plot development of the original text.这七个维度进行设置，每个维度包含1至2个问题，并引入测谎题目以确保问卷的准确性。具体的问题设置可见附录\ref{}。考虑到评估人员一次性阅读太长的文本进行评估会对其主观感受造成影响，我们将小说选段和剧本选段的字数限制在1000个token左右，同时从每篇小说-剧本中随机挑选若干个选段对进行评估，以保证评估结果能够反映小说改编剧本的整体情况。
同时，我们招募评估人员并对他们进行专业培训。每位评估人员在填写问卷之前需仔细阅读原始小说，并对比分析两种方法基于该章节改编的两个电影剧本选段A和B回答调研问卷。调查问卷所有问题的选项只有A、B和全部选择，全不选择，评估人员不会获知剧本的具体来源，他们只需要根据题目选择符合自身感受的选项。最后，我们汇总问卷结果并按照下列公式计算各个维度的赢率：

On the other hand, 人类评估有可能代入过多的主观考虑导致评估结果波动很大从而影响评估结果的准确性，很多文本生成工作考虑使用GPT-4对长文本进行评估\citep{}。following this，这里我们也通过将人类评估的调查问卷输入给GPT-4对我们生成的剧本进行评估以获得GPT-4的评估结果，我们将GPT-4得到的评估结果与人工评估结果一起展示。

\paragraph{Baselines} 我们将我们的方法与ROLLING，CHAPTER，Dramatron\citep{}和Wawa Writing Tool\citep{}进行比较。ROLLING是通过将小说按照GPT-4o-mini最大输入长度16k切分成rolling windows要求GPT-4o-mini逐段将小说改编成剧本的baseline。CHAPTER是要求GPT-4o-mini将小说的每一章都改编成剧本的baseline。Dramatron是一个从logline中生成剧本的方法，为了与我们的方法进行比较，我们将小说的大纲作为输入让Dramatron生成剧本。Wawa Writing Tool是一个现有的AI写作工具，我们使用它的小说转剧本功能将我们收集的小说转换成剧本与我们的方法进行比较。






==> documents/scratch.tex <==
\begin{table}[t]

\centering
% \footnotesize % 可以根据需要调整为 \scriptsize 或其他适当的大小
\caption{Comparison of Novel-Script Pairs and Associated Movie Data}

\scalebox{0.9}{
\begin{tabular}{l|r|r|r|r|r|r}
\toprule

\textbf{Data Type}  & \textbf{Novel-Script Pairs} & \textbf{Average Novel Word Count} & \textbf{Average Script Word Count} & \textbf{Average Movie Reviews} & \textbf{Average Movie Rating} & \textbf{Genres}  \\
\midrule
Test Novel-Script Data Pair      & 3                           & 180050.3                          & 25131.7                           & 4944.7                         & 6.0                           & Suspense / Sci-Fi / Romance / Love / Drama / Crime  \\
\multirow{2}{*}{Niche Novel-Script Data Pair     & 10                          & 159487.4                          & 28434.7                           & 62526.9                        & 6.5                           & Suspense / Crime / Comedy / Love / Romance / Sci-Fi / Adventure / Thriller / Biography / History / Drama}  \\
Popular Novel-Script Data Pair   & 10                          & 133995.9                          & 29736.7                           & 757127.0                       & 8.98                          & Sci-Fi / Thriller / Drama / Suspense / Action / Crime / War / Biography / History  \\ 

\bottomrule
\end{tabular}
}
\label{tab:dataset}
\end{table}
